Doing More by Doing Less: How Structured Partial Backpropagation Improves Deep Learning Clusters

Many organizations employ compute clusters equipped with accelerators such as GPUs and TPUs for training deep learning models in a distributed fashion. Training is resource-intensive, consuming significant compute, memory, and network resources. Many prior works explore how to reduce training resource footprint without impacting quality, but their focus on a subset of the bottlenecks (typically only the network) limits their ability to improve overall cluster utilization. In this work, we exploit the unique characteristics of deep learning workloads to propose Structured Partial Backpropagation(SPB), a technique that systematically controls the amount of backpropagation at individual workers in distributed training. This simultaneously reduces network bandwidth, compute utilization, and memory footprint while preserving model quality. To efficiently leverage the benefits of SPB at cluster level, we introduce JigSaw, a SPB aware scheduler, which does scheduling at the iteration level for Deep Learning Training(DLT) jobs. We find that JigSaw can improve large scale cluster efficiency by as high as 28\%.

==> acmart-primary/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> acmart-primary/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

==> future_directions.tex <==
\section{Future Work and Discussion}
\begin{myitemize}
    \item \textbf{Space Multiplexing}: As seen in Table:~\ref{table:sbp_promise}, \sbpAcrnm{}
      reduces the GPU memory usage of the DLT job as well. This opens opportunity for space
      multiplexing, which can further improve the cluster utilization. While the V100 GPUs in our
      cluster did not have support for space-partitioning, we plan to investigate if this can help
      when using A100 GPUs~\cite{mig}.  
      %Space multiplexing on GPUs can be enabled using CUDA\_STREAMS, however, we found significant overhead in enabling this at fine granularity of iterations.          
    \item \textbf{Dynamic \sbpAcrnm{}}: Recent works have proposed different stages of DNN
      training~\cite{frankle2020early,leclerc2020regimes}, with each stage having different needs.
      At present \sbpAcrnm{} is static in terms of work distribution across workers. 
      % There's always a worker which does the full backpropagation. 
      We plan to relax this constraint and let
      \name{} also change the work distribution based on the training stage of a job. %in the future. 
      %of the workers according to the training stage
      %they are in and contention in the cluster.
    \item \textbf{\sbpAcrnm{} with other compression schemes}: Communication
      optimization techniques like Top-K, Random-K, Quantization can be used along with \sbpAcrnm{},
      leading to better performance in low bandwidth setting. We plan to study the convergence and
      cluster utilization.  
    \item \textbf{Warm Start}: Recent works~\cite{frankle2020early} have shown that early stage of
      DNN training is quite crucial with respect to the final quality. To improve the quality of
      model with \sbpAcrnm{}, we plan to study a warm start strategy, where for initial few iterations
      the model is trained with standard SGD.     
\end{myitemize}


==> results.tex <==
\section{Results}
\subsection{\sbpAcrnm{ }  effect on Model Quality}
We first present empirical results on the convergence of popular deep learning models when using
\sbpAcrnm{} while training.  We consider models from a number of domains including computer vision,
NLP etc. and also consider models of different complexity (i.e., depth or number of layers). 

For CV, we considered image classification
with CIFAR10 and CIFAR100 datasets and a number of DNN families
(ResNet, VGG, GoogLeNet, and DenseNet). We used SGD with momentum and
$10^{-4}$ weight decay as our optimizer configuration. We tried 3
learning rates for each model and picked the one attaining best
accuracy. For NLP, we selected models for classification on the MR
dataset~\cite{mr} and language modeling on
WikiText~\cite{wikitext}. We use 4 workers, each running on an NVIDIA
V100 GPU, for all the experiments.

% \noindent\textbf{Accuracy.}
 We present a comparison of the accuracy achieved when using
\sbpAcrnm{} vs. a baseline where models are trained using standard distributed SGD optimization in Table~\ref{table:sbp_accuracy}.
% All the models in this case were run using 4 workers for a fixed number of epochs and we present
% accuracy on validation data. All the CV models (Resnet, VGG, GoogLeNet, DenseNet) were trained
% on CIFAR-10 while the NLP models were trained on WikiText, MR dataset. Our results show that using \sbpAcrnm{} has minimal effect on accuracy with 1-2\% difference from standard SGD training. 

%We also show the convergence across epochs for ResNet18, GoogleNet and VGG19 when trained on CIFAR-10 and observe that SPB makes very similar progress to the baseline. All the models in this case were run using 4 workers for a fixed number of epochs and we present accuracy on test data. 
% \textbf{Results}:
Our results from Table~\ref{table:sbp_accuracy} shows that there is a minimal effect on the accuracy achieved when models are trained with \sbpAcrnm{}. Even though the DNN early layers are getting updated by fewer workers, model convergence is not significantly impacted.
%updated less frequently,can be attributed 
We attribute this behavior of \sbpAcrnm{} to the fact that early layers
converge faster than later layers, and thus require fewer gradient
descent steps. This has also been observed by previous
work~\cite{freezeOut,freezeTraining}. 

Further, %% we see that for a given task using SPB on a more complex
%% model does not significantly impact accuracy. However, we do
we note that 
using \sbpAcrnm{} for a more complex task could lead to a bigger difference in
% \begin{wraptable}[15]{r}{6.9cm}%[!t]
\begin{table}%{H}{6.9cm}%[!t]
  % \scriptsize
%\begin{minipage}{0.5\columnwidth}
  \small
  \centering
\begin{tabular}{c|c| c|c}
  \toprule
  % \hline
  % \multirow{2}{*}{\textbf{Model}} &
    % \multicolumn{1}{c|}{\textbf{Structured Backprop Pruning}} &
    % \multicolumn{1}{c|}{\textbf{No Dropping}} \\
   \multirow{2}{*}{\textbf{Dataset}} &
    \multirow{2}{*}{\textbf{Model}} & \textbf{Accuracy} & \textbf{Accuracy}\\
    & & \textbf{\sbpAcrnm{}} & \textbf{SGD} \\
%      \textbf{Dataset}& \textbf{Model}& \textbf{Accuracy w \sbpAcrnm{}} & \textbf{Accuracy w/o \sbpAcrnm{}}\\
    \midrule
    \multirow{7}{*}{CIFAR10} & ResNet18 & 93.96 & 94.02 \\
    & ResNet34 & 93.81 & 94.96 \\
    % & MobileNet & - & - \\
    & DenseNet121 & 94.18 & 94.35 \\
    & GoogleNet & 94.07 & 93.83 \\
    % & LeNet & - & - \\
    & VGG16 & 91.93 & 92.35 \\
    \hline
    \multirow{3}{*}{CIFAR100} & ResNet18 & 71.31 & 72.83 \\
    & ResNet34 & 69.94 & 71.2 \\
    % & DenseNet121 & - & - \\
    \hline
    \multirow{2}{*}{MR} & CNNText & 77.12 & 77.35 \\
    & LSTMText & 78.02 & 80.23 \\
    \hline
    WikiText 2 & LSTM & 105* & 103* \\
    \bottomrule
    \end{tabular}
%  \end{minipage}
    \caption{Comparison of maximum accuracy of various models w/o SPB. *Perplexity is reported for language model on WikiText.} %\shivaram{Please mark what the columns mean. Accuracy of 105 doesn't make
    % sense? Is it some other unit?}}
    \label{table:sbp_accuracy}
    %\vspace*{-5mm}
  \end{table}
%Further, %% we see that for a given task using SPB on a more complex
%% model does not significantly impact accuracy. However, we do
%we note that 
%using \sbpAcrnm{} for a more complex task could lead to a bigger difference in
accuracy (though still under 2\%). For example, with ResNet18, the accuracy difference due to
\sbpAcrnm{} increases from 0.06\% to 1.52\% as we go from CIFAR10 to CIFAR100. This we believe can
be overcome by warm up epochs, where for initial $N$ epochs we train the model using the full
gradient from all the workers. 

\begin{figure*}[b]
  \centering
  \subfloat[\label{fig:conv}Convergence of ResNet18 on CIFAR10 as we vary the number of workers.]{\includegraphics[width=0.3\linewidth]{imgs/resnet18acc.eps}}
  \hspace{0.5in}
  \subfloat[\label{fig:makespan}Makespan comparison of DLT schedulers on a simulated 35 GPU
  cluster.]{\includegraphics[width=0.3\linewidth]{imgs/GPU_35_Makespan.eps}}
  \caption{}
\end{figure*}

Figure~\ref{fig:conv} shows the convergence of ResNet18 model when varying the number of workers on the
CIFAR10 dataset while using SPB. We maintain a batch size of 128 per worker. 
From the figure we see that as we increase the number of workers it takes
more iterations to converge to the best accuracy. Our theory also suggests this in terms of the 
$log(k)$ factor in the convergence rate for $k$ workers, albeit for convex functions. 
Also, we find that the maximum accuracy achieved using 8 workers is slightly lesser than that 
achieved with 4 workers. We believe that this could be related to using a larger batch size in this
setting. We discuss ways in discussion section to close this gap in accuracy. 



\subsection{\name: Prototype SBP aware Scheduler}
Even though \sbpAcrnm{} can save compute resources as well as bandwidth, existing state of the art DLT schedulers~\cite{gandiva,tiresias,SLAQ,optimus} cannot opportunistically use any resources saved by the gradient approximations as they are unaware of gradient approximation schemes used by jobs.
% Thus, they treat training jobs as black boxes requiring fixed
% resources, and cannot opportunistically use any resources saved by the approximations.  % Second, while a number of cluster schedulers have
% been proposed to allocate resources across training jobs in a
% cluster~\cite{gandiva,tiresias,SLAQ,optimus}, existing schedulers are unaware of gradient approximation schemes used by jobs. Thus, they treat training jobs as black boxes requiring fixed
% resources, and cannot opportunistically use any resources saved by the approximations. 
 Our vision is to build a DLT scheduler which improves the cluster efficiency without compromising the quality of DLT jobs. 
 In that direction, we present a preliminary result that showcases the potential benefits from a \sbpAcrnm{}-aware DLT job scheduler
 Compared with Gandiva~\cite{gandiva} and
 Tiresias~\cite{tiresias} on public trace of 480 DLT jobs simulated to run on a 35 GPU cluster, we
 see that a \sbpAcrnm{}-aware scheduler can finish all jobs in 400 mins, while Tiresias, Gandiva
 takes ~780 and ~820 mins respectively (Figure~\ref{fig:makespan}).
% can be seen in~\Cref{fig:makespan} our scheduler is able to finish all jobs in 400 mins, while Tiresias, Gandiva takes ~780 and ~820 mins respectively. 

%\begin{wrapfigure}[10]{l}{8cm}%[!t]
%  \centering
%  \includegraphics[width=0.7\linewidth]{imgs/resnet18acc.eps}
%  \vspace*{-5mm}
%  \caption{\shivaram{to fix} Structured Partial Backpropagation}
%  \label{fig:resnet18acc}
%  %\vspace*{-5mm}
%\end{wrapfigure}
%
\begin{wrapfigure}[11]{l}{8cm}%[!t]
 \centering
 \includegraphics[width=0.7\linewidth]{imgs/GPU_35_Makespan.eps}
 \vspace*{-5mm}
 \caption{[Simulation]: Makespan comparison of DLT schedulers across 35 GPU cluster. Backpropagation}
 \label{fig:makespan}
 %\vspace*{-5mm}
\end{wrapfigure}

%  \begin{figure*}
%   \centering
% \subfloat[\textbf{W1} 35 GPU Cluster]{\includegraphics[width=0.5\columnwidth]{imgs/GPU_35_Makespan.eps}}
%   \subfloat[\textbf{W1} 60 GPU Cluster]{\includegraphics[width=0.5\columnwidth]{imgs/GPU_60_Makespan.eps}}
% \subfloat[ \textbf{W2} :45 GPU Cluster]{\includegraphics[width=0.5\columnwidth]{imgs/workload_2_makespan.eps}}
% \vspace*{-3mm}
%   \caption{\label{fig:makespan}
%        [Workload 1] Comparison of makespan of JigSaw with different DNN Job Scheduler on varying scale of GPU Cluster}
% \vspace*{-6mm}
%   \end{figure*}

%while a number of cluster schedulers have
%been proposed to allocate resources across training jobs in a
%cluster~\cite{gandiva,tiresias,SLAQ,optimus}, existing schedulers are unaware of gradient approximation schemes used by jobs. Thus, they treat training jobs as black boxes requiring fixed
%resources, and cannot opportunistically use any resources saved by the approximations.



==> sched-algo.tex <==
%!TEX root = example_paper.tex
\begin{figure}
  \vspace*{-5mm}
  % \begin{figure}
  \begin{minipage}{\columnwidth}
    \begin{algorithm}[H]
    % \scriptsize
    \small
    % \begin{multicols}{2}
      \begin{algorithmic}[1]
        \State \textbf{Procedure} \textsc{SPBAwareScheduler}($\mathcal{T}, \mathcal{M}, \mathcal{I}$)
        \begin{ALC@g}
        \STATE{\textbf{Input}: $\mathbb{T}$: Current Task List, $\mathcal{M}$: Number of machines, $\mathcal{T}$: Scheduling Interval}
        \STATE{\textbf{Output}: Task-Schedule $\mathcal{S}$ for $\mathcal{M}$ machines}
        \STATE{TaskQ: Priority Queue of Tasks}
        % \STATE{t = $0$ // start time is $0$}
        \FOR{$task \in \mathbb{T}$} 
            \STATE{score = normalize(t.mem $\times$ t.duration $\times$ t.compute)}
            \STATE{TaskQ.insert($task$, score)} \label{line:taskqueueend}
        \ENDFOR 
      %   \STATE{RT-Space $\mathcal{S}$ = CreateSpace($\mathcal{M}$, $\mathcal{I}$)}
        \WHILE {TaskQ is not empty}
            \STATE{$task$ = TaskQ.pop() // Pop task with max score} \label{line:taskpop}
            \FOR{d $\in$ M} \label{line:bestdvc}
              \IF {migration\_needed}
              \STATE{m\_t = GetMigrationTime(task.model\_size, d)} 
              \ELSE 
              \STATE{m\_t = 0}
              \ENDIF  
            % \STATE{if needs_migration == True:}
              % \If{needs\_migration}
              \STATE{feasible\_t = t + m\_t} \label{line:migrationTime}
              \STATE{start\_time[d] = d.GetEarliestStartTime(feasible\_t )}  
            \ENDFOR
            \STATE{// Pick device with earliest start time }
            \STATE{assigned\_d = $argmin_{\text{d}}$ start\_time[d]} \label{line:placetask}
          %   \STATE{status = PlaceTask($\mathcal{S}$, $t$)} \label{line:placetask}
            \IF{if assigned\_d != None}                                          
            \STATE{AssignTaskToDevice($\mathcal{S}$, task, assigned\_d)} \label{line:assignDvc}eval
            \STATE{AddNextIterationTasks(TaskQ)} \label{line:nextIterationFlush}
          %   \STATE{UpdateTasks(TaskQ, $\mathcal{S}$, $t$)} \label{line:updatetask}
            \ELSE 
                \STATE{continue}
            \ENDIF
        \ENDWHILE 
        \STATE{\textbf{return} $\mathcal{S}$ // task schedule}
        \end{ALC@g} 
      \end{algorithmic}
    % \end{multicols}
      \caption{SPB Aware Scheduler}
  \label{alg:taskplacement}
\end{algorithm}
\end{minipage}
\vspace*{-4mm}
% \end{figure}
\end{figure}


==> scheduler.tex <==
\section{Scheduling SBP Jobs}
\label{section:sched}

In this section we describe the design of a DL scheduler that can improve cluster utilization
and makespan by taking advantage of the resources saved by SBP. We begin by describing why current
DL schedulers are ineffective and then discuss some of the key challenges in developing a new
scheduler. Finally we present the design of our SBP-aware scheduler.

\begin{figure}[!t]
	% \centering
  \subfloat[Gang Scheduling with SBP]{\includegraphics[width=0.5\columnwidth]{imgs/sched-job-level.pdf}}
  \hspace{0.1in}
    \subfloat[Iteration-level scheduling with SBP]
    {\includegraphics[width=0.48\columnwidth]{imgs/sched-iter-level.pdf}}
	\caption{\label{fig:job-schedule} Example of gang scheduling versus iteration-level 
  scheduling for DLT jobs with SBP. Gang scheduling, which operates at a job-level, 
  cannot utilize the resources saved due to SBP.}
  \vspace{-0.15in}
\end{figure}

\subsection{Scheduling DL workloads}
% short intro on how schedulers work.
In shared clusters used for DL, users typically submit jobs to a
centralized scheduler~\cite{philly}. Each job is annotated with the
number of GPUs required and the amount of memory required per-GPU. The
scheduler uses a \emph{policy} to determine which jobs get access to
which GPUs. Scheduling policies take into account job characteristics
like time taken per iteration, model size etc., and aim to maximize
cluster utilization~\cite{gandiva} or fairness~\cite{tiresias} etc.

%\begin{wrapfigure}{r}{0.4\textwidth}
%    \includegraphics[width=0.9\linewidth]{imgs/dlt-job.pdf}
%  \caption{Deep learning training task DAG of job $J$ with arrows indicating dependencies. 
%  Tasks of iteration 2 can run 
%  only after all tasks of iteration 1 have completed and so on.}
%    \label{fig:dlt-job}
%\end{wrapfigure}

% gang scheduling is used by existing schedulers. if resources for all tasks are not available then
% job waits in queue
% recent work tiresias allows shorter jobs to progress by preemption but still have gang scheduling
Existing schedulers typically use \emph{gang scheduling} for placing
distributed DL training jobs. Using gang scheduling implies that all
the workers for a job are started at the same time; thus if say for a
$8$ worker job, only 4 GPUs are available, then the job continues to
wait till 4 more GPUs become free. This often leads to significant
queue wait times for short running jobs~\cite{philly}. Recent work has
proposed pre-empting longer running jobs to improve waiting times and
fairness~\cite{tiresias}, but gang scheduling is nevertheless used.

% SBP cannot be used by gang scheudlers
Despite these recent improvements, gang scheduling based schedulers
fundamentally cannot capitalize on the resources saved using
SBP. Figure~\ref{fig:job-schedule}(a) shows an example where worker0
for Job1 finishes an iteration in 0.3s whereas worker2 takes
1s. Existing schedulers are not able to capitalize on this and can
only schedule the next job after the longest-running worker finishes.

\subsection{SBP-Aware Scheduler}
In this paper we propose designing a new scheduling approach for DL
jobs where we weaken the gang-scheduling requirement and instead
schedule every iteration at each worker independently, and each worker
relinquishes its GPUs as soon as its iteration is done.  With this
approach as shown in Figure~\ref{fig:job-schedule}(b), once worker0
finishes for Job1 we can immediately start a worker for Job2. This
removes GPU idling from Figure~\ref{fig:job-schedule}(a) thereby
improving cluster utilization.

% weaken the requirement using PS arch.
% need to rethinking scheduler to be more fine-grained where each worker for a job can be placed
% independently
% more flexibility in time -> reduces makespan
% reduction from backprop, spatial mux -> multiple smaller jobs can run
Using our approach improves utilization due to two main reasons:
\begin{itemize}
  \item By scheduling at the granularity of an iteration at each worker we are able to do more
    efficient \emph{time multiplexing}, thereby capitalizing on the backward pass time savings from SBP. 
  \item SBP also reduces peak memory
    requirements. This means that we can do more efficient \emph{space
      multiplexing} where multiple jobs' workers can share a GPU at
    the same time.
\end{itemize}

%Along with time savings, 

% Challenges to doing this
 %  Locality --> ML model iteration update hard to do time sharing
 %  Spatial sharing of GPUs --> not easy to control what fraction of GPU is used. Nee to control
%  memory, compute etc. 
\noindent\textbf{Challenges.} However there are a number of challenges
in designing a scheduler that can achieve the above listed
benefits. Performing fine-grained scheduling could mean that the next
iteration for a job could be on a different machine than the previous
iteration. Migrating the DL computation graph 
% \adarsh{model most work use strategy of saving model parameters and sending.}
%\aditya{params as at the PS? so no need to move?}
%  and model parameters
to a new machine
involves network overheads that need to be taken into account. Further
existing accelerators like GPUs provide limited support for running
multiple jobs simultaneously. Co-locating jobs could lead to a
slowdown and we find that the degree to which jobs are slowed down
varies based on the model characteristics.\footnote{Empirically
  measured slowdowns for co-resident models on
  GPUs is presented in the
  Appendix.}.
  %commonly-used 
  %state-of-the-art 

\subsection{Scheduling Algorithm}
We propose a new scheduler that takes into account both of the above
overheads when making scheduling decisions. To do this we first
perform a profiling step when a job is submitted and collecting
information such as the model size, memory required etc. 

\textbf{ILP Formulation}: Given the above input, we first attempted an
ILP formulation to solve for a schedule: specifically, given a set of jobs that are
present in the queue, we derive a scheduling plan for an upcoming
interval $\mathcal{I}$ (e.g., 60s). The objective is to minimize the
finish time of the last job, i.e., minimize makespan. The constraints
here include ensuring that compute and memory resources are not 
oversubscribed at any GPU and that dependencies across DL iterations are
maintained (next iteration of a job does not start at a worker until
all workers finish the previous iteration). We present the full
formulation in Appendix. %~\ref{sec:appendix_ilp}.

In practice, for a GPU cluster of say 60 machines and hundreds of DL
training jobs, the above formulation led to around $10^{6}$ variables and
constraints. Using a commercial solver for this problem we found that
generating the optimal schedules takes more than one minute when we
have a scheduling interval ($\mathcal{I}$) of 60 seconds, thus making
the ILP unsuitable in practice.

% \input{sched-algo}

\minisection{Online Algorithm} Thus, we consider a heuristic
scheduling scheme to achieve minimal makespan, i.e., minimize the
finish time of the last task/worker among all training jobs.  We
present our scheduling algorithm in \Cref{alg:jigsaw-scheduler}.  The
scheduler periodically computes a schedule for an fixed interval
(scheduling interval $\mathcal{I}$) by placing ``tasks'' in a
2-dimensional space of resources, namely, GPU device and time. Here a
``task'' captures the a worker of a particular job running a single
iteration. The scheduler also takes into account, task dependencies
across iterations. 
% \aditya{this was the first mention of tasks --
  % defined it here}
%By computing schedules periodically, the scheduler can be used to assign
%resources to jobs in an online fashion (as they arrive to the scheduler).
%The scheduler tries to minimize makespan and maximize cluster utilization by maintaining a

The scheduler maintains a priority queue, where tasks are queued with
their priority defined as product of memory usage, compute usage and duration
(\Cref{line:taskqueueend}). The idea of defining priority as product
of resources is inspired from bin packing
heuristics~\cite{binPacking}--tasks with longer running times or
consuming more memory would be harder to fit in the resource space.

%As long as the priority queue (TaskQ) is non-empty, 
The task with the highest priority $t$ is removed from the queue
(TaskQ) and the scheduler computes the earliest start time for $t$ on
each device. This calculation involves accounting for the two
overheads mentioned before. To account for the network overhead from
migrating a worker to a new device, we add the expected transfer time
to the running time $t$ (\Cref{line:migrationTime}). This gives preference for a worker to stay on
the same device. To account for co-resident model sharing overheads,
we use profiling data to derive the fraction of GPU compute ($c_{t}$)
that is necessary for a task to avoid slowdown. We then filter our
device list to only include GPUs which have adequate compute resources
available. We discuss how profiling is done in detail in Appendix.

% \aditya{we should include the full pseudocode for how
%   overheads are culated, and for getearlieststarttime to the appendix,
%   and include a reference here.}

%taking into account $t$'s dependencies and resource availability on
%the device.
%The device with the earliest time is chosen for the task
%(\Cref{line:bestdvc}).
%the scheduling plan along with device resource
%usage for the duration of task $t$ is then updated (\Cref{line:assignDvc}).
Once a task is placed at the chosen device (\Cref{line:assignDvc}), we check if this was
the last task of the iteration. If yes, we enqueue tasks for the next iteration. % this job. 
%This logic is handled in
%(\Cref{line:nextIterationFlush}). 
Thus, tasks of iteration $i+1$ are
scheduled only after all tasks of iteration $i$ have been scheduled,
hence, adhering to the task dependencies across iterations. 
%\aditya{the heuristic does not talk about locality and spatial multiplexing, which were brought out in 3.2}



% Solution -> Optimization program, expensive to solve
% Heuristic -> account for network overhead and also spatial sharing overheads.
\begin{figure*}[b]
  \centering
  \subfloat[\label{fig:conv}Convergence of ResNet18 on CIFAR10 as we vary the number of workers.]{\includegraphics[width=0.3\linewidth]{imgs/resnet18acc.eps}}
  \hspace{0.5in}
  \subfloat[\label{fig:makespan}Makespan comparison of DLT schedulers on a simulated 35 GPU
  cluster.]{\includegraphics[width=0.3\linewidth]{imgs/GPU_35_Makespan.eps}}
  \caption{}
\end{figure*}

